Appearance-based Gaze Estimation With Deep Learning: A Review and Benchmark

Human gaze provides valuable information on human focus and intentions, making it a crucial area of research. Recently, deep learning has revolutionized appearance-based gaze estimation. However, due to the unique features of gaze estimation research, such as the unfair comparison between 2D gaze positions and 3D gaze vectors and the different pre-processing and post-processing methods, there is a lack of a definitive guideline for developing deep learning-based gaze estimation algorithms. In this paper, we present a systematic review of the appearance-based gaze estimation methods using deep learning. Firstly, we survey the existing gaze estimation algorithms along the typical gaze estimation pipeline: deep feature extraction, deep learning model design, personal calibration and platforms. Secondly, to fairly compare the performance of different approaches, we summarize the data pre-processing and post-processing methods, including face/eye detection, data rectification, 2D/3D gaze conversion and gaze origin conversion. Finally, we set up a comprehensive benchmark for deep learning-based gaze estimation. We characterize all the public datasets and provide the source code of typical gaze estimation algorithms. This paper serves not only as a reference to develop deep learning-based gaze estimation methods, but also a guideline for future gaze estimation research. The project web page can be found at https://phi-ai.buaa.edu.cn/Gazehub.

==> Authors/bios.tex <==
Yihua Cheng received the B.S. degree in computer science from Beijing University of Posts and Telecommunications in 2017, and Ph.D. degree in computer science from Beihang University in 2022. He is now a Postdoctoral Researcher with University of Birmingham, UK. His research interests include gaze estimation, hand pose estimation, object pose estimation and human-robot interaction.
	
Haofei Wang received the B.S. degree with distinction from Zhejiang University in 2013, and Ph.D. degree in electronic and computer engineering from the Hong Kong University of Science and Technology in 2020. He is now a Postdoctoral Researcher with the Pengcheng Laboratory, Shenzhen, China. His research interests include eye tracking, gaze estimation, human-computer interaction and mixed reality.

Yiwei Bao currently pursuing the Ph.D. degree with the State Key Laboratory of Virtual Reality Technology and Systems, School of Computer Science and Engineering, Beihang University. His research interests include computer vision and human gaze analysis.

Feng Lu received the B.S. and M.S. degrees in automation from Tsinghua University, in 2007 and 2010, respectively, and the Ph.D. degree in information science and technology from The University of Tokyo, in 2013. He is currently a Professor with the State Key Laboratory of Virtual Reality Technology and Systems, School of Computer Science and Engineering, Beihang University. His research interests include computer vision, human-computer interaction and augmented intelligence.

